Semi-invariant Riemannian metrics in hydrodynamics

Many models in mathematical physics are given as non-linear partial differential equation of hydrodynamic type; the incompressible Euler, KdV, and Camassa--Holm equations are well-studied examples.A beautiful approach to well-posedness is to go from the Eulerian to a Lagrangian description.Geometrically it corresponds to a geodesic initial value problem on the infinite-dimensional group of diffeomorphisms with a right invariant Riemannian metric. By establishing regularity properties of the Riemannian spray one can then obtain local, and sometimes global, existence and uniqueness results. There are, however, many hydrodynamic-type equations, notably shallow water models and compressible Euler equations, where the underlying infinite-dimensional Riemannian structure is not fully right invariant, but still semi-invariant with respect to the subgroup of volume preserving diffeomorphisms. Here we study such metrics. For semi-invariant metrics of Sobolev $H^k$-type we give local and some global well-posedness results for the geodesic initial value problem. We also give results in the presence of a potential functional (corresponding to the fluid's internal energy). Our study reveals many pitfalls in going from fully right invariant to semi-invariant Sobolev metrics; the regularity requirements, for example, are higher. Nevertheless the key results, such as no loss or gain in regularity along geodesics, can be adopted.

==> definitions.tex <==
%\usepackage{amsmath,amssymb}
% \usepackage{relsize}

% -- General math stuff
\DeclareMathOperator{\real}{Re}
\DeclareMathOperator{\imag}{Im}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\divv}{div}
\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\rot}{\curl}
\DeclareMathOperator{\tr}{tr}
\newcommand{\ee}{\mathrm{e}}
\newcommand{\ii}{\mathrm{i}}
\newcommand{\pair}[1]{\left\langle #1 \right\rangle}
\newcommand{\poisson}[1]{\{ #1 \}}
\newcommand{\inner}[1]{\langle\!\langle #1 \rangle\!\rangle}
\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\vect}[1]{\boldsymbol{#1}}

% -- Differential operators
% \newcommand{\ud}{\operatorname{d}}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\udd}{\,\ud}
\newcommand{\uud}{\,\ud}
\newcommand{\pd}{\partial}

% -- Standard sets
\newcommand{\RR}{{\mathbb R}}
\newcommand{\CC}{{\mathbb C}}
\newcommand{\ZZ}{{\mathbb Z}}
\newcommand{\NN}{{\mathbb N}}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\disk}{\mathbb{D}}
\newcommand{\DD}{\disk}
\newcommand{\TT}{\mathbb{T}}

% -- Geometry
\newcommand{\vol}{\mu}
\newcommand{\Vol}{\mathrm{Vol}}
\newcommand{\met}{\mathsf{g}}
\newcommand{\Diff}{\mathrm{Diff}}
\newcommand{\Xcal}{\mathfrak{X}}
\newcommand{\Diffvol}{{\Diff_{\vol}}}
\newcommand{\Xcalvol}{{\Xcal_{\vol}}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\LieD}{\mathcal{L}}
\newcommand{\interior}{\mathrm{i}}
\newcommand*\incl{\imath}
\newcommand{\Dens}{\mathrm{Dens}}
\newcommand{\Prob}{\mathrm{Prob}}
\newcommand{\Jac}{\mathrm{Jac}}
\newcommand{\dist}{\mathrm{dist}}


% -- Lie groups/algebras
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\Ad}{Ad}
\newcommand*\GL{\mathrm{GL}}
\newcommand*\id{\mathrm{id}}
\newcommand*\gl{\mathfrak{gl}}
\newcommand*\SO{\mathrm{SO}}
\newcommand*\OO{\mathrm{O}}
\providecommand{\so}{\mathfrak{so}}
\newcommand*\SU{\mathrm{SU}}
\newcommand*\su{\mathfrak{su}}
\newcommand*\SE{\mathrm{SE}}
\newcommand*\se{\mathfrak{se}}
\newcommand*\g{\mathfrak{g}}

% -- Commonly used operators
\newcommand{\iunit}{\mathrm{i}}


% -- LOCAL COMMANDS
\newcommand{\eps}{\varepsilon}

\def\o{\circ}
\def\X{\mathfrak X}
\def\al{\alpha}
\def\be{\beta}
\def\ga{\gamma}
\def\de{\delta}
\def\ep{\varepsilon}
\def\ze{\zeta}
\def\et{\eta}
\def\th{\theta}
\def\io{\iota}
\def\ka{\kappa}
\def\la{\lambda}
\def\rh{\rho}
\def\si{\sigma}
\def\ta{\tau}
\def\ph{\varphi}
\def\ch{\chi}
\def\ps{\psi}
\def\om{\omega}
\def\Ga{\Gamma}
\def\De{\Delta}
\def\Th{\Theta}
\def\La{\Lambda}
\def\Si{\Sigma}
\def\Ph{\Phi}
\def\Ps{\Psi}
\def\Om{\Omega}
\def\i{^{-1}}
\def\x{\times}
\def\p{\partial}
\let\on=\operatorname


% \usepackage{aliascnt}

%  % ---- plain ----
% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}[theorem]{Proposition}

%  % ---- definition ----
% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{remark}[theorem]{Remark}



